Buffered Streaming Edge Partitioning

Addressing the challenges of processing massive graphs, which are prevalent in diverse fields such as social, biological, and technical networks, we introduce HeiStreamE and FreightE, two innovative (buffered) streaming algorithms designed for efficient edge partitioning of large-scale graphs. HeiStreamE utilizes an adapted Split-and-Connect graph model and a Fennel-based multilevel partitioning scheme, while FreightE partitions a hypergraph representation of the input graph. Besides ensuring superior solution quality, these approaches also overcome the limitations of existing algorithms by maintaining linear dependency on the graph size in both time and memory complexity with no dependence on the number of blocks of partition. Our comprehensive experimental analysis demonstrates that HeiStreamE outperforms current streaming algorithms and the re-streaming algorithm 2PS in partitioning quality (replication factor), and is more memory-efficient for real-world networks where the number of edges is far greater than the number of vertices. Further, FreightE is shown to produce fast and efficient partitions, particularly for higher numbers of partition blocks.

==> preamble.tex <==
\bibliographystyle{plainurl}
\newcommand{\scaleFactorSmall}{0.49}
\newcommand{\imgScaleFactorSmall}{1}
\newcommand{\capPositionSmall}{-.4cm}
\newcommand{\afterCapSmall}{-.45cm}
\usepackage[normalem]{ulem}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{framed,enumitem} 
\usepackage[lineno]{algorithm}
\usepackage{numprint}
\npdecimalsign{.}
\npthousandsep{\,}
\usepackage[noend]{algpseudocode}
\usepackage{colortbl}
\usepackage{amsbsy}
\usepackage{mathtools}


